Operational Semantics with Hierarchical Abstract Syntax Graphs

This is a motivating tutorial introduction to a semantic analysis of programming languages using a graphical language as the representation of terms, and graph rewriting as a representation of reduction rules. We show how the graphical language automatically incorporates desirable features, such as alpha-equivalence and how it can describe pure computation, imperative store, and control features in a uniform framework. The graph semantics combines some of the best features of structural operational semantics and abstract machines, while offering powerful new methods for reasoning about contextual equivalence. All technical details are available in an extended technical report by Muroya and the author and in Muroya's doctoral dissertation.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{P. Bahr (Ed.): 11th International Workshop on\\
Computing with Terms and Graphs (TERMGRAPH 2020)\\
EPTCS 334, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.334.1}{10.4204/EPTCS.334.1}}
\pdfoutput=1

